DSPO: Direct Semantic Preference Optimization for Real-World Image Super-Resolution

Recent advances in diffusion models have improved Real-World Image Super-Resolution (Real-ISR), but existing methods lack human feedback integration, risking misalignment with human preference and may leading to artifacts, hallucinations and harmful content generation. To this end, we are the first to introduce human preference alignment into Real-ISR, a technique that has been successfully applied in Large Language Models and Text-to-Image tasks to effectively enhance the alignment of generated outputs with human preferences. Specifically, we introduce Direct Preference Optimization (DPO) into Real-ISR to achieve alignment, where DPO serves as a general alignment technique that directly learns from the human preference dataset. Nevertheless, unlike high-level tasks, the pixel-level reconstruction objectives of Real-ISR are difficult to reconcile with the image-level preferences of DPO, which can lead to the DPO being overly sensitive to local anomalies, leading to reduced generation quality. To resolve this dichotomy, we propose Direct Semantic Preference Optimization (DSPO) to align instance-level human preferences by incorporating semantic guidance, which is through two strategies: (a) semantic instance alignment strategy, implementing instance-level alignment to ensure fine-grained perceptual consistency, and (b) user description feedback strategy, mitigating hallucinations through semantic textual feedback on instance-level images. As a plug-and-play solution, DSPO proves highly effective in both one-step and multi-step SR frameworks.

==> sec/sup.tex <==




\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|l|>{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}}
\toprule
\multicolumn{1}{l|}{\textbf{Dataset}} & \textbf{Method} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{DISTS$\downarrow$} & 
\textbf{NIQE$\downarrow$}&
\textbf{MUSIQ$\uparrow$} & \textbf{MANIQA$\uparrow$} & \textbf{CLIPIQA$\uparrow$} \\ \midrule
\multirow{5}{*}{DrealSR}   
&Pre-trained&27.92 	&0.7835 	&0.2968 	&\bluebf{0.2165} 	&6.4902 	&64.65 	&0.5895 	&0.6963 \\
&SFT&\bluebf{27.95} 	&\bluebf{0.7899} 	&\bluebf{0.2961} 	&0.2240 	&6.6098 	&64.46 	&0.5960 	&0.6914 \\
&DDPO&\bluebf{27.95} 	&0.7817 	&0.3021 	&0.2273 	&6.6240 	&\bluebf{65.60} 	&0.6018 	&0.6861\\
&Diff-DPO&27.41 	&0.7768 	&0.3105 	&0.2279 	&\redbf{6.4352} 	&65.23 	&\bluebf{0.6026} 	&\bluebf{0.6964} \\
&DSPO&\redbf{27.97} 	&\redbf{0.7919} 	&\redbf{0.2869} 	&\redbf{0.2150} 	&\bluebf{6.4409} 	&\redbf{65.82} 	&\redbf{0.6057} 	&\redbf{0.7043} \\  \midrule
\multirow{5}{*}{RealSR}
&Pretain&25.15 	&0.7341 	&\bluebf{0.2921} 	&\bluebf{0.2128} 	&\bluebf{5.6476} 	&69.09 	&0.6331 	&0.6693 \\
&SFT&25.11 	&\bluebf{0.7363} 	&0.3000 	&0.2222 	&5.7962 	&68.55 	&0.6252 	&\bluebf{0.6746} \\
&DDPO&25.08 	&0.7257 	&0.2993 	&0.2232 	&5.6654 	&\bluebf{69.14} 	&\bluebf{0.6438} 	&0.6479 \\
&Diff-DPO&\bluebf{25.16} 	&0.7278 	&0.3025 	&0.2249 	&6.0459 	&68.36 	&0.6232 	&0.6558 \\
&DSPO&\redbf{25.23} 	&\redbf{0.7368} 	&\redbf{0.2826} 	&\redbf{0.2099} 	&\redbf{5.5974} 	&\redbf{69.42} 	&\redbf{0.6503} 	&\redbf{0.6819} \\
\midrule
\multirow{5}{*}{DIV2K-Val}
&Pre-trained&\redbf{23.72}	&0.6108	&\bluebf{0.2941}	&\redbf{0.1976}	&\bluebf{4.7097}	&\bluebf{67.97}	&0.6148	&\bluebf{0.6683}\\
& SFT&23.56	&\bluebf{0.6155}	&0.2999	&0.2284	&4.8700	&65.49	&0.6135	&0.6144\\
& DDPO&23.20	&0.6059	&0.3059	&0.2119	&4.8094	&67.15	&0.5823	&0.6666\\
& Diff-DPO&23.44	&0.6082	&0.3038	&0.2137	&4.7131	&\bluebf{67.97}	&\bluebf{0.6209}	&0.6602\\
& DSPO &\bluebf{23.68}	&\redbf{0.6202}	&\redbf{0.2930}	&\bluebf{0.2018}	&\redbf{4.7000} 	&\redbf{68.34}	&\redbf{0.6259}	&\redbf{0.6818}\\ 
\bottomrule
\end{tabular}}
\caption{Performance comparison of  DSPO with baselines on one-step SR framework based on RealSR, DRealSR, and DIV2K-val. `Diff-DPO' is the abbreviation for Diffusion-DPO.}
\label{tab:single}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Performance Comparison of DSPO and Other Baseline Method}
A comparison of the experimental performance of the DSPO and other baseline methods is conducted based on the results from Tables \ref{tab:single} and \ref{tab:multi}. The findings indicate that the DSPO model achieves optimal performance in both one-step SR and multi-step SR frameworks.
\section{Ablation Study on Parameter Settings}
An ablation study is presented that examines the impact of various $\beta$ parameter settings on performance metrics within the RealSR dataset. The results indicate that setting $\beta$ to 8000 yields an overall better effect, significantly enhancing the effectiveness of super-resolution tasks within the one-step SR framework as Table\ref{tab:Ablationbeta} shown.
\section{Visual Comparison of DSPO and Baseline Methods}
A visual comparison between the DSPO method and other baseline approaches is presented, highlighting performance differences across various super-resolution frameworks. The visual results demonstrate that DSPO produces more realistic detail textures while effectively mitigating issues such as artifacts and blurriness as Fig\ref{fig:Visualization_sup}.


\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|l|>{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}
                >{\centering\arraybackslash}p{1.25cm}}
\toprule
\multicolumn{1}{l|}{\textbf{Dataset}} & \textbf{Method} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{DISTS$\downarrow$} & 
\textbf{NIQE$\downarrow$}&
\textbf{MUSIQ$\uparrow$} & \textbf{MANIQA$\uparrow$} & \textbf{CLIPIQA$\uparrow$} \\ \midrule
\multirow{5}{*}{DRealSR}
&Pre-trained&27.21 	&0.7598 	&0.3380 	&0.2535 	&6.5110 	&61.16 	&0.5877 	&0.6675 \\
&SFT&27.48 	&\bluebf{0.7601} 	&0.3450 	&0.2401 	&6.5091 	&60.36 	&0.5862 	&0.6679 \\
&DDPO&27.10 	&0.7599 	&0.3310 	&0.2521 	&6.4510 	&62.11 	&0.6058 	&\bluebf{0.6712} \\
&Diff-DPO&\bluebf{27.94} 	&0.7465 	&\bluebf{0.3254} 	&0.2464 	&\bluebf{6.3921} 	&\bluebf{63.13} 	&\bluebf{0.6100} 	&0.6698 \\
&DSPO &\redbf{28.06} 	&\redbf{0.7611} 	&\redbf{0.3156} 	&\redbf{0.2355} 	&\redbf{6.3723} 	&\redbf{64.27} 	&\redbf{0.6111} 	&\redbf{0.6821}  \\  \midrule
\multirow{5}{*}{RealSR} 
&Pre-tained&24.76 	&0.7005	&0.3170	&0.2385	&5.7237	&68.91 	&0.6218	&\bluebf{0.6535}\\
&SFT&\bluebf{25.00} 	&0.7098	&\bluebf{0.3001}	&\bluebf{0.2325}	&5.6959	&67.05 	&0.6105	&0.6424\\
&DDPO&24.86 	&\bluebf{0.7111}	&0.3098	&0.2412	&\bluebf{5.6099}	&68.90 	&0.6115	&0.6428\\
&Diff-DPO&24.84 	&0.7089	&0.3211	&0.2329	&5.68795	&\bluebf{69.03} 	&\bluebf{0.6258}	&0.6515\\
&DSPO &\redbf{25.23} 	&\redbf{0.7144}	&\redbf{0.2912}	&\redbf{0.2208}	&\redbf{5.5961}	&\redbf{69.56} 	&\redbf{0.6423}	&\redbf{0.6688} \\ \midrule
\multirow{5}{*}{DIV2K-Val}
&Pre-trained &23.63 &0.5794 &0.3227 &0.2152 &4.8352 &65.26 &0.6143 	&\bluebf{0.6723} \\
&SFT &\redbf{24.00} &0.5628 &0.3209 &\bluebf{0.2097} &\bluebf{4.7007} &66.93 &0.6028 &0.6697 
\\
&DDPO &23.18 &0.5898 &0.3192 &0.2139 &4.7773 &\bluebf{67.81} &0.6144 &0.6520 
\\
&Diff-DPO &23.35 	&\bluebf{0.5906} 	&\bluebf{0.3188} 	&0.2161 	&4.8855 	&65.98 	&\bluebf{0.6222} 	&0.6721 \\
&DSPO  &\bluebf{23.99} 	&\redbf{0.6074} 	&\redbf{0.3122} 	&\redbf{0.2050} 	&\redbf{4.6613} 	&\redbf{67.86} 	&\redbf{0.6283} 	&\redbf{0.6758} 
\\\bottomrule
\end{tabular}}
\caption{Performance comparison of  DSPO with baselines on muti-step SR framework based on RealSR, DRealSR, and DIV2K-val. `Diff-DPO' is the abbreviation for Diffusion-DPO.}
\label{tab:multi}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\begin{tabular}{c|l|cccccccc}
\toprule
\multicolumn{1}{l|}{\textbf{Dataset}} & \textbf{$\beta$} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{DISTS$\downarrow$} & 
\textbf{NIQE$\downarrow$}&
\textbf{MUSIQ$\uparrow$} & \textbf{MANIQA$\uparrow$} & \textbf{CLIPIQA$\uparrow$} \\ \midrule
\multirow{4}{*}{DrealSR}
&500&27.51 	&0.7749 	&0.3203 	&0.2362 	&6.4776 	&64.85 	&0.5792 	&0.6599 \\
&5000&27.82 	&0.7823 	&0.2992 	&0.2276 	&6.5444 	&64.17 	&0.5856 	&0.6740 \\ %ok
&8000&27.97 	&0.7919 	&0.2869 	&0.2150 	&6.4409 	&65.82 	&0.6057 	&0.7043 \\ %ok
&4000000&27.13 	&0.7589 	&0.3290	&0.2356 	&5.9197 	&66.07 	&0.5906 	&0.7036 \\ \midrule %ok
%27.5107 	0.7749 	0.3203 	0.2362 	154.9454 	6.4776 	64.8505 	0.5792 	0.6599 
% 27.8182	0.7823	0.2992	0.2276	150.98416	6.5444	64.1678	0.5856	0.674
% &DSPO &28.06 	&0.7611 	&0.3156 	&0.2355 	&6.3723 	&64.27 	&0.6111 	&0.6821  \\  \midrule
% \multirow{5}{*}{DIV2K-Val}
% &Pre-trained\\
% &SFT\\
% &DDPO\\
% &Diff-DPO\\
% &DSPO  \\\bottomrule
\end{tabular}
\caption{
Ablation study on the impact of different $\beta$ parameter settings on performance metrics in the DrealSR dataset.}
\label{tab:Ablationbeta}
\end{table*}
% \end{document}



\begin{figure*}[!]

  \vspace{5pt} % 增加垂直间距
    \begin{subfigure}[b]{\linewidth}
      \centering
      \includegraphics[width=\linewidth]{figure/human_realsr.jpg}
  \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
      \centering
      \includegraphics[width=\linewidth]{figure/osediff_real_supp.jpg}
  \end{subfigure}
      \begin{subfigure}[b]{\linewidth}
      \centering
      \includegraphics[width=\linewidth]{figure/seesr_real.jpg}
  \end{subfigure}
  
  \centering

  % \vspace{5pt} % 增加垂直间距
  \caption{Visualization comparison of DSPO and other baseline methods on the human annotator method (Top), and the automatic IQA model Method with one-step SR framework (Middle) and multi-step SR framework (Bottom).}
  % \caption{Visualization comparison of DSPO and other baseline methods on the Human Annotator Method (Top), and the automatic IQA Model Method with one-step SR framework (Middle) and multi-step SR framework (Bottom).}
  \label{fig:Visualization_sup}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table*}[!t]
% \centering
% \begin{tabular}{c|l|>{\centering\arraybackslash}p{1.25cm}
%                 >{\centering\arraybackslash}p{1.25cm}
%                 >{\centering\arraybackslash}p{1.25cm}
%                 >{\centering\arraybackslash}p{1.25cm}
%                 >{\centering\arraybackslash}p{1.25cm}
%                 >{\centering\arraybackslash}p{1.25cm}
%                 >{\centering\arraybackslash}p{1.25cm}
%                 >{\centering\arraybackslash}p{1.25cm}}
% \toprule
% \multicolumn{1}{l|}{\textbf{Datast}} & \textbf{Method} & \textbf{PSNR$\uparrow$} & \textbf{SSIM$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{DISTS$\downarrow$} & 
% \textbf{NIQE$\downarrow$} & \textbf{MUSIQ$\uparrow$} & \textbf{MANIQA$\uparrow$} & \textbf{CLIPIQA$\uparrow$} \\ \midrule
% \multirow{4}{*}{DrealSR}     
% &Pre-trained &27.92 	&0.7835 	&0.2968 	&0.2165 	&6.4902 	&64.65 	&0.5895 	&0.6963  \\
% &Perception&25.36 	&0.7157 	&0.3528 	&0.2427 	&\redbf{5.9302} 	&\redbf{68.64} 	&\redbf{0.6334} 	&\redbf{0.7080}\\
% & Fidelity&\redbf{28.57} 	&\redbf{0.8024} 	&\redbf{0.2855} 	&\redbf{0.2149} 	&6.5870 	&62.76 	&0.5726 	&0.6538 \\
% & United &\bluebf{27.97} 	&\bluebf{0.7919} 	&\bluebf{0.2869} 	&\bluebf{0.2150} 	&\bluebf{6.4409} 	&\bluebf{65.82} 	&\bluebf{0.6057} 	&\bluebf{0.7043} \\\midrule
% \multirow{4}{*}{RealSR}
% &Pre-trained&25.15 	&0.7341 	&0.2921 	&0.2128 	&5.6476 	&69.09 	&0.6331 	&0.6693 \\
% &Perception&22.55 	&0.6615 	&0.3297 	&0.2270 	&\redbf{5.3484} 	&\redbf{70.19}	&\redbf{0.6633} 	&\bluebf{0.6768}  \\
% & Fidelity&\redbf{25.33} 	&\redbf{0.7395} 	&\bluebf{0.2870} 	&\bluebf{0.2109} 	&5.9373 	&67.07 	&0.6177 	&0.6304\\
% &United&\bluebf{25.23}	&\bluebf{0.7368} 	&\redbf{0.2826} 	&\redbf{0.2099} 	&\bluebf{5.5974} 	&\bluebf{69.42} 	&\bluebf{0.6503} 	&\redbf{0.6819}\\ \bottomrule
% \end{tabular}
% \caption{The ablation study on different different optimization objectives. `All' represents the use of both perception and fidelity metrics. The best and second
% best results of each metric are highlighted in \redbf{red} and \bluebf{blue}, respectively.}
% \label{tab:abmetric}
% \end{table*}
